Computational Mechanics of Input-Output Processes: Structured transformations and the $\epsilon$-transducer

Computational mechanics quantifies structure in a stochastic process via its causal states, leading to the process's minimal, optimal predictor---the $\epsilon$-machine. We extend computational mechanics to communication channels between two processes, obtaining an analogous optimal model---the $\epsilon$-transducer---of the stochastic mapping between them. Here, we lay the foundation of a structural analysis of communication channels, treating joint processes and processes with input. The result is a principled structural analysis of mechanisms that support information flow between processes. It is the first in a series on the structural information theory of memoryful channels, channel composition, and allied conditional information measures.

==> oharp.tex <==
\makeatletter
\newcommand{\orharp}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \rvectfill\crcr\noalign{\kern-1.2pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\rvectfill{%
  $\m@th\smash-\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightharpoonup$}

\newcommand{\olharp}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \lvectfill\crcr\noalign{\kern-1.2pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\lvectfill{%
  $\m@th\smash\leftharpoonup\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
\mkern-7mu\smash-$}

\newcommand{\olrharp}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \lrvectfill\crcr\noalign{\kern-1.2pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\lrvectfill{%
  $\m@th\smash\leftharpoonup\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightharpoonup$}

\newcommand{\orharplow}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \rvectfill\crcr\noalign{\kern-1.9pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\rvectfill{%
  $\m@th\smash-\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightharpoonup$}

\newcommand{\olharplow}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \lvectfill\crcr\noalign{\kern-1.9pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\lvectfill{%
  $\m@th\smash\leftharpoonup\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
\mkern-7mu\smash-$}

\newcommand{\olrharplow}[1]{%
  \vbox{\m@th \ialign {##\crcr
  \lrvectfill\crcr\noalign{\kern-1.9pt \nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}
\def\lrvectfill{%
  $\m@th\smash\leftharpoonup\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\smash-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightharpoonup$}
\makeatother
